LLM Benchmarking with LLaMA2: Evaluating Code Development Performance Across Multiple Programming Languages

The rapid evolution of large language models (LLMs) has opened new possibilities for automating various tasks in software development. This paper evaluates the capabilities of the Llama 2-70B model in automating these tasks for scientific applications written in commonly used programming languages. Using representative test problems, we assess the model's capacity to generate code, documentation, and unit tests, as well as its ability to translate existing code between commonly used programming languages. Our comprehensive analysis evaluates the compilation, runtime behavior, and correctness of the generated and translated code. Additionally, we assess the quality of automatically generated code, documentation and unit tests. Our results indicate that while Llama 2-70B frequently generates syntactically correct and functional code for simpler numerical tasks, it encounters substantial difficulties with more complex, parallelized, or distributed computations, requiring considerable manual corrections. We identify key limitations and suggest areas for future improvements to better leverage AI-driven automation in scientific computing workflows.

==> codes_examples/code_generation.tex <==

%
% Gode Generation - Numerical Integration - Python
%

\begin{lstlisting}[language=python,caption=Generated python code for the numerical integration using scipy.,label=python:integration:scipy,escapechar=|, float=false]
import numpy as np
from scipy.integrate import quad

# define the function sin(x)
def f(x):
    return np.sin(x)

# define the limits of integration
a = -np.pi
b = 2*np.pi/3

# compute the integral using quad
result, error = quad(f, a, b)

print("The area between -π and 2/3π for sin(x) is: ", result)
\end{lstlisting}

\begin{lstlisting}[language=python,caption=Generated python code for the numerical integration using a Riemann sum.,label=python:integration:riemann,escapechar=|, float=!htbp]
import numpy as np

# define the function sin(x)
def f(x):
    return np.sin(x)

# define the limits of integration
a = -np.pi
b = 2*np.pi/3

# define the number of intervals for the Riemann sum
n = 1000

# compute the width of each interval
dx = (b - a) / n

# initialize the sum
sum = 0

# compute the Riemann sum
for i in range(n):
    x = a + i * dx
    sum += f(x) * dx

print("The area between -π and 2/3π for sin(x) is: ", sum)
\end{lstlisting}


==> codes_examples/testing.tex <==
%
% Testing - Numerical Integration - C++
%

\begin{lstlisting}[language=c++,caption=Generated unit tests for the \cpp numerical integration example.,label=cpp:testing,escapechar=|, float=false]
#include <gtest/gtest.h>
#include "riemann_sum.h" // assume the code is in a header file called riemann_sum.h

TEST(RiemannSumTest, SimpleTest) {
  // Test the Riemann sum for a simple case
  double a = 0.0;
  double b = M_PI / 2.0;
  int n = 1000;
  double expected_result = 1.0; // exact value of the integral
  double tolerance = 1e-3; // tolerance for the comparison

  double result = riemann_sum(a, b, n);
  EXPECT_NEAR(result, expected_result, tolerance);
}

TEST(RiemannSumTest, NegativeLimitsTest) {
  // Test the Riemann sum for a case with negative limits
  double a = -M_PI / 2.0;
  double b = 0.0;
  int n = 1000;
  double expected_result = -1.0; // exact value of the integral
  double tolerance = 1e-3; // tolerance for the comparison

  double result = riemann_sum(a, b, n);
  EXPECT_NEAR(result, expected_result, tolerance);
}

TEST(RiemannSumTest, LargeNTest) {
  // Test the Riemann sum for a large number of intervals
  double a = 0.0;
  double b = M_PI;
  int n = 100000;
  double expected_result = 2.0; // exact value of the integral
  double tolerance = 1e-6; // tolerance for the comparison

  double result = riemann_sum(a, b, n);
  EXPECT_NEAR(result, expected_result, tolerance);
}

int main(int argc, char **argv) {
  ::testing::InitGoogleTest(&argc, argv);
  return RUN_ALL_TESTS();
}

\end{lstlisting}

==> codes_examples/translation.tex <==
%
% Code Translation - Numerical Integration - Matlab to R
%
\begin{lstlisting}[language=R,caption=Transalted matlab code to R for the numerical integration example.,label=matlab:R:translation,escapechar=|, float=false]
# Define the limits of integration
a <- -pi
b <- 2/3 * pi

# Compute the area using the definite integral
area <- integrate(sin(x), a, b)

# Print the result
cat("Area:", area, "\n")

\end{lstlisting}
